Deep Learning for Quality Control of Subcortical Brain 3D Shape Models

We present several deep learning models for assessing the morphometric fidelity of deep grey matter region models extracted from brain MRI. We test three different convolutional neural net architectures (VGGNet, ResNet and Inception) over 2D maps of geometric features. Further, we present a novel geometry feature augmentation technique based on a parametric spherical mapping. Finally, we present an approach for model decision visualization, allowing human raters to see the areas of subcortical shapes most likely to be deemed of failing quality by the machine. Our training data is comprised of 5200 subjects from the ENIGMA Schizophrenia MRI cohorts, and our test dataset contains 1500 subjects from the ENIGMA Major Depressive Disorder cohorts. Our final models reduce human rater time by 46-70%. ResNet outperforms VGGNet and Inception for all of our predictive tasks.

==> intro/intro.tex <==
In recent years, connectomics has become a popular form of analysis for neuroimaging data. The construction of structural connectomes, derived from diffusion MRI data, involves multiple pre-processing steps, each of which can be performed in a variety of different ways. It is often unclear, however, what the best combination of choices is, for specific dataset or application, or what their effect is on the resulting data. Due to the ongoing work on each of these steps, the number of possible processing pipelines is growing at a combinatorially remarkable rate.

There is also a very large number of graph summary statistics and derived features. While each has its purpose, merits, and historical derivation, it is again unclear which of these features capture the most relevant information for specific applications.

It is thus useful to investigate the effects of pre-processing choices on resulting connectivity models, and various information measures for their relative information content. It is difficult to assess each possible pipeline due to their number, but we believe it is important to narrow down the space of options. In this paper, we present reproducibility and simple classification task results for three diffusion models, with generated streamlines using two different methods, using seven different parcellations and four different normalization schemes, generating nine different graph features (\figurename{\ref{overview_fig}}). While it is unlikely there exists a single best pipeline for all data for all research objectives, in the present work we provide data on qualities we believe to be necessary, though not sufficient for inclusion in rigorous analyses, for the specific tasks we analyze.

As a basic sanity check for the usefulness of structural network generation methods and features, we propose to use pair-wise classification accuracy (PACC) as a multivariate potentially non-linear supplement to the usual intraclass correlation coefficient used in test-retest datasets. The task at hand, given a particular set of network features, is to separate network pairs arising from different scans of the same subject from pairs from different subjects. As additional validation, we evaluated accuracy in a sex classification task, using each of the network feature sets assessed before. 

Our main result is as follows: in terms of reproducibility and our simple classification tasks, probabilistic tracking using either a Constrained Spherical Deconvolution local model \cite{tournier2007robust} or the Constant Solid Angle \cite{aganj2010reconstruction}  method gave the best combination of pairwise classification and mean ICC. This result is consistent across three datasets of healthy adult test-retest scans, with both a low and moderate number of diffusion angles (30 and 62). In terms of predicting poor performance in another classification task, the combination of low ICC and low pairwise classification accuracy appears to predict poor performance while either of these measures alone does not; this was also found consistently across datasets. Though we conjecture that such a "useless feature" identification would generalize to other classification tasks, this result is not sufficient to guarantee the generalization. 




==> pipe/pipe.tex <==
\section{Structural Connectomics Pipelines}

We abstract the connectome construction process to the following steps (in order of processing): fitting a local diffusion model, reconstructing tracts, fitting a cortical parcellation and counting streamline endpoint pairs, normalization, and building connectome features (see \figurename{\ref{overview_fig}}). We first describe the options we assessed at each stage, then the methods by which we assessed them. For the remainder of the paper we denote a set of connectomes as $\{C^i_j\}$, where $j$ is an index of a subject and $i$ is an index of an image. 

\subsection{Reconstruction models and tractography}

\label{reconstruction}


We consider three widely-used methods for reconstruction  of white matter architecture \cite{daducci2014quantitative}. The \textbf{Diffusion Tensor} model (DTI) is by far the most well known, in that it is often incorrectly synonymous with diffusion-weighted imaging. DTI is also the simplest model, simply fitting an ellipsoidal diffusion pattern at each voxel. The \textbf{Constant Solid Angle} model (CSA) \cite{aganj2010reconstruction} produces orientation density functions that are generalizations of the ellipsoidal diffusion tensor to any continuous spherical function. This particular method is regularized and uses spherical harmonics to parameterize spherical functions. \textbf{Constrained Spherical Deconvolution} (CSD) \cite{tournier2007robust} models dominant tract directions as delta functions on the sphere convolved with a response kernel. The deconvolution recovers these directions from an estimated empirical ODF.

Once local models of fiber orientation have been constructed, a whole brain tractography reconstruction is applied. Here there are two general categories, \textbf{deterministic} tracking, which takes only the principle fiber direction, and \textbf{probabilistic}, which uses the full ODF and not simply the mode.


\subsection{Parcellations and Network Construction}
\label{parcellations}

There is a wide variety of parcellation choices. These have a non-trivial effect on the resulting graphs and derived graph measures \cite{van2010comparing}, and also, as we show here, on the consistency of those measures. We test the following parcellations, which were chosen based on their popularity and to represent a variety of scales: Desikan-Killiany (DK) \cite{desikan2006automated}, Destrieux \cite{destrieux2010automatic}, and the Lausanne 2008 (at five different scales) \cite{hagmann2008mapping}. We recorded the number of streamlines having endpoints in each pair of labels for each parcellation, using these counts as edge weights in each constructed connectome. The normalization of connectivity matrices also may be useful prior to any analysis (\cite{hagmann2007mapping}, \cite{bassett2011conserved}). We use the following three normalization schemes along with no normalization at all: mean, maximum, and binary normalization with zero threshold. 

%  \[
%  a^{mean}_{kl}= \frac{a_{kl} \left(\begin{array}{c}n\\2\end{array}\right)}{\sum_{k',l'} a_{k'l'}}~~~~
%  a^{max}_{kl}=\frac{a_{kl}}{\max_{k'l'} a_{k'l'}} ~~~~
%  a^{binary}_{kl}= \left\{\begin{array}{cc}1 & a_{kl} > 0\\ 0 &~~~~~ \text{otherwise}~~\end{array}\right.
%  \] 
%  where $a_{kl}$ is an edge weight.

% Normalization by mean of all matrix elements 
% \begin{equation}
% w^{by~sum}_{ij}=\frac{a_{ij}}{\sum_{ij}{a_{ij}}}.
% \end{equation}

% Normalization by maximum alone.
% \begin{equation}
% w^{by~max}_{ij}=\frac{a_{ij}}{\max_{i,j}a_{ij}}.
% \end{equation}

%\textbf{}

\subsection{Network features}
\label{features}

For each connectome and each normalization we build ``bag of edges" vectors from the upper triangle of the adjacency matrix. In addition, we calculate eight network metrics for each node: \textbf{weighted degrees}, or strength; \textbf{closeness}, \textbf{betweenness} and \textbf{eigenvector centralities}; \textbf{local efficiency}; \textbf{clustering coefficient}; and \textbf{weighted number of triangles} around node. We choose these features because they are well-described and reflect different structural properties of connectomes \cite{rubinov2010complex}. We also calculate PageRank for each node. Introduced in 1998 by Brin and Page \cite{pagerank_original} this metric roughly estimates probability that a random walk on the network will be observed at particular node.

\subsection{Pairwise features}
\label{pairs}

Each normalization and set of features described above defines a mapping from connectome space to feature space $C \rightarrow f(C)$. As our goal is to check how well this mapping separates connectomes in it, we propose various pairwise features. For each set of connectome features in question we make all possible pairs of connectome features -- ($f(C^{i_1}_{j_1}), f(C^{i_2}_{j_2})$). For each pair, we assign a binary target variable -- 1 if connectomes are from the same subject ($j_1 = j_2$), 0 -- if they are from different subjects ($j_1 \neq j_2$). Finally, for each pair we build a vector of three features, describing their difference $\|f(C_1) - f(C_2) \|$ according to $l_1$, $l_2$ and $l_{\infty}$ norms.

\subsection{Classification models and validation}

We use linear classifiers for pairwise  and sex classification problems: logistic regression, SVM with linear kernel and stochastic gradient descent (SGD) with modified Huber loss. We scale features with standard scaling and apply elastic-net regularization for each of the classifiers.

We measure model performance and accuracy, in a two-step validation procedure. First, for each dataset, we perform hyperparameter grid search based on a 5-fold cross-validation with a fixed random state for reproducibility. For each model, we varied the overall regularization parameter, $l_1$-ratio and number of iterations for SGD. Then we evaluate the best parameters on 50 train/test splits with fixed different random states (test size was set to 20\% of data). We characterize each connectome building pipeline and feature by mean pairwise/sex classification accuracy on these 50 test splits.

\subsection{Reproducibility measure}

As a reproducibility measure for connectome mapping, we use the Intraclass Correlation Coefficient \cite{shrout1979intraclass} between measurements taken at different time points: 
$$
ICC = \frac{BMS-WMS}{BMS + (k-1)WMS},
$$
where BMS is the between-subject mean sum of squares, WMS is the within-subject mean sum of squares, and $k$ is the number of scans per subject. For each pipeline and derived set of features we exclude features with no variation and calculate mean ICC value for remaining features, thus characterizing this pipeline by one ICC value. 

